The one clean qubit model without entanglement is classically simulable

Entanglement has been shown to be necessary for pure state quantum computation to have an advantage over classical computation. However, it remains open whether entanglement is necessary for quantum computers that use mixed states to also have an advantage. The one clean qubit model is a form of quantum computer in which the input is the maximally mixed state plus one pure qubit. Previous work has shown that there is a limited amount of entanglement present in these computations, despite the fact that they can efficiently solve some problems that are seemingly hard to solve classically. This casts doubt on the notion that entanglement is necessary for quantum speedups. In this work we show that entanglement is indeed crucial for efficient computation in this model, because without it the one clean qubit model is efficiently classically simulable.

==> chris.tex <==
\section{Definitions and notation}\label{sec:defs}

We begin by formally introducing the central object of the proofs that follow -- the `control-unitary' gate. Informally, this is a 2-qubit gate that is controlled on one qubit, in some basis, and acts on the other qubit with a unitary that depends upon the state of the first qubit. 
\begin{definition}[2-qubit control unitary]
A \emph{2-qubit control unitary} is a unitary $\CU{A}{B}{C}$ such that, if $\mathcal{A}$ is the basis (for 1 qubit) $\{\ket{a}, \ketp{a}\}$, then
\[
	\CU{A}{B}{C}: \begin{matrix} \quad & \ket{a}\ket{\psi} \mapsto \ket{a}B\ket{\psi} \\ \quad & \ketp{a}\ket{\psi} \mapsto \ketp{a}C\ket{\psi}
	\end{matrix}.
\]
$\CU{A}{B}{C}$ has eigenvectors $\ket{a}\ket{b}, \ket{a}\ketp{b}, \ketp{a}\ket{c}, \ketp{a}\ketp{c}$, where $\mathcal{B} = \{\ket{b},\ketp{b}\}$ and $\mathcal{C} = \{\ket{c}, \ketp{c}\}$ are the eigenbases of $B$ and $C$, respectively. We will draw such a gate as in Figure \ref{fig:CU}. Since these gates will always be 2-qubit gates, we will write $\UC{A}{B}{C}$ to represent a control unitary controlled on the second qubit, and acting on the first. 
\end{definition}

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=1.0]{diagrams/control_unitary.pdf}
\caption{A $\CU{A}{B}{C}$ gate.}
\label{fig:CU}
\end{center}
\end{figure}


Some straightforward observations follow. 

\begin{observation}
Suppose we have the control-unitary $\CU{A}{B}{B'}$, and $[B,B']=0$. Then
\begin{itemize}
\item $\CU{A}{B}{B'}$ is diagonal in the $\mathcal{A} \otimes \mathcal{B}$ basis.
\item For $B = \unitary{e^{i\theta_1}}{0}{0}{e^{i\theta_2}}$ and $B' = \unitary{e^{i\phi_1}}{0}{0}{e^{i\phi_2}}$, we have $\CU{A}{B}{B'} = \UC{B}{A}{A'}$, where $A = \unitary{e^{i\theta_1}}{0}{0}{e^{i\phi_1}}$ and $A' = \unitary{e^{i\theta_2}}{0}{0}{e^{i\phi_2}}$.
\end{itemize}
\end{observation}

\begin{observation}
Suppose we have the control-unitary $\CU{A}{B}{B'}$, and $B' = e^{i\theta}B$ for some angle $\theta$. Then
\begin{itemize}
\item $\CU{A}{B}{B'} = \CU{A}{e^{i\phi}B}{e^{i\varphi}B} = A \otimes B$ for $A = \unitary{e^{i\theta}}{0}{0}{e^{i\phi}}$ in the $\mathcal{A}$ basis. 
\end{itemize}
\end{observation}


We note that there are three `types' of control-unitary:
\chris{Need to finish this part / move it somewhere else / make it less formal}
\begin{itemize}
\item \emph{Ordinary} : $\mathcal{C} = \{ \CU{A}{B}{C} \}$ \note{Example? CNOT?}
\item \emph{Phase} : $\mathcal{P} = \{ \CU{A}{B}{B'} : [B,B']=0, B \neq e^{i\phi} B' ~\forall \phi \in [0,2\pi] \}$ \note{Example? CZ?}
\item \emph{Separate/Product} : $\mathcal{S} = \{ \CU{A}{B}{B'} : B = e^{i\phi} B' \text{ for some } \phi \in [0,2\pi] \}$ \note{Example? }
\end{itemize}

Finally, we define precisely what we mean when we say that a circuit (or the unitary corresponding to that circuit) has a product eigenbasis.
\begin{definition}[Product eigenbasis]
We say that a unitary $U$ has a \emph{product eigenbasis} when there is an eigenbasis of $U$ such that every eigenvector in the basis is a product state. 

More precisely, an $n$-qubit unitary $U$ has a product eigenbasis if it can be written as 
\[
    U = \sum_{i \in 2^n} \alpha_i \proj{\psi_i}
\]
for coefficients $\alpha_i \in \mathbb{C}$, and $\ket{\psi_i}$ is a product state for all $i$.
\end{definition}
~\\\\
The following Lemma will be used throughout: 
\begin{lemma}\label{lem:product}
Suppose we have a state on $|C| + |T|$ qubits, $\ket{\psi}_C\ket{\phi}_T = \sum_x \alpha_x \ket{x}_C \ket{\phi}_T$, that is acted upon by a unitary $U = \sum_x \proj{x} \otimes U_x$:
\[
	\sum_x \alpha_x \ket{x}_C \ket{\phi}_T \mapsto U \left(\sum_x \alpha_x \ket{x}_C \ket{\phi}_T\right) = \sum_x \alpha_x \ket{x}_C U_x\ket{\phi}_T.
\]
If the state $\ket{\psi}\ket{\phi}$ is an eigenvector of $U$ with eigenvalue $e^{i\theta}$, then for all $\alpha_x \neq 0$, $\ket{\phi}_T$ is also an eigenvector of $U_x$ with eigenvalue $e^{i\theta}$. 
\end{lemma}
\begin{proof}
We have
\[
	\sum_x \alpha_x \ket{x}_C U_x\ket{\phi}_T = e^{i\theta}\left( \sum_x \alpha_x \ket{x}_C \ket{\phi}_T  \right)
\]
for some phase $\theta$. Write $\ket{\phi} = \sum_y \beta_y \ket{y}$. Then 
\[
\sum_{x,y} \alpha_x \beta_y \ket{x}_C U_x\ket{y}_T = e^{i\theta}\sum_{x,y} \alpha_x \beta_y \ket{x} \ket{y}.
\]
In particular, this means that for every $x$, $y$,
\[
\ket{x}U_x\ket{y} = e^{i\theta}\ket{x}\ket{y}
\]
Since $\{\ket{x}\ket{y}, \ket{x}\ket{y}\}_{x,y}$ forms a orthonormal basis over both registers, this condition can only hold if $U_x\ket{y} = e^{i\theta}\ket{y}$ for all $x,y$.  
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Main proofs}
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Structure of single 2-qubit gates and simple circuits}
%%%%%%%%%%%%
\begin{lemma}\label{lem:single_2_qubit}
Suppose we have a 2-qubit unitary with a product eigenbasis. Then this unitary must be a control unitary $\CU{A}{B}{C}$ (or $\UC{A}{B}{C}$) for some choice of $\mathcal{A}, B$, and $C$. 
\end{lemma}
\begin{proof}
Since it is product, the eigenbasis must have the form $\{\ket{\psi_0}\ket{\phi_0}, \ket{\psi_1}\ket{\phi_1}, \ket{\psi_2}\ket{\phi_2}, \ket{\psi_3}\ket{\phi_3}\}$. However, as we will now show, the possible choices for the $\psi_i$ and $\phi_i$ are heavily constrained. We can pick an eigenbasis by arbitrarily choosing a basis vector $\ket{a^\perp}\ket{c}$, and then choose the subsequent basis vectors under the constraint that they must be orthogonal to all previous basis vectors -- see Figure \ref{fig:bases}.
\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.65]{diagrams/basis_choices.pdf}
\caption{All possible choices of product eigenbases for a 2-qubit unitary.}
\label{fig:bases}
\end{center}
\end{figure}
By inspection, one can see that all choices of bases consistent of a single 1-qubit basis on one of the qubits, and two 1-qubit bases on the other qubit, each corresponding to one of the possible basis vectors on the first qubit. Hence, the only basis choice we can have is 
\[
\{ \ket{a}\ket{b}, \ket{a}\ket{b^\perp}, \ket{a^\perp}\ket{c}, \ket{a^\perp}\ket{c^\perp} \},
\]
for some 1-qubit bases $\{\ket{a},\ket{a^\perp}\}, \{\ket{b},\ket{b^\perp}\}, \{\ket{c},\ket{c^\perp}\}$ (up to swapping the first and second qubit). Hence, the unitary $U$ must be of the form 
\[
\proj{a}\left(e^{i\theta_1} \proj{b}+ e^{i\theta_2}\proj{b^\perp}\right) + \proj{a^\perp}\left( e^{i\phi_1} \proj{c}+ e^{i\phi_2}\proj{c^\perp}\right),
\]
where $e^{i\theta_1}, e^{i\theta_2}, e^{i\phi_1},  e^{i\phi_2}$ are the eigenvalues associated with each eigenvector. Written in the $\mathcal{A} = \{\ket{a},\ket{a^\perp}\}$ basis, this is 
\[
\begin{pmatrix}
B & 0 \\
0 & C
\end{pmatrix},
\]
corresponding to a controlled $B/C$ gate: if qubit 1 is in state $\ket{a}$, then the unitary $B = e^{i\theta_1}\proj{b}+e^{i\theta_2}\proj{b^\perp}$ is applied, else if qubit 1 is in state $\ket{a^\perp}$, then unitary $C = e^{i\phi_1}\proj{c}+e^{i\phi_2}\proj{c^\perp}$ is applied. Hence, the unitary must be a control unitary $\CU{A}{B}{C}$.
\end{proof}
%%%%%%%%%%%%

%%%%%%%%%%%%
\begin{lemma}\label{lem:single_qubit_gates}
Suppose we have the following circuit: 

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=1.0]{diagrams/lemma2.pdf}
%\caption{}
\label{fig:lemma2}
\end{center}
\end{figure}

Then its corresponding unitary has a product eigenbasis in the following cases:
\begin{itemize}
\item If $[QBV, QCV] \neq 0$, and $U$ and $P$ are diagonal in the $\mathcal{A}$ basis.
\item If $[QBV, QCV] = 0$.
\item If $B = e^{i \phi}C$ for some angle $\phi$.
\end{itemize}
\end{lemma}
\begin{proof}
We begin by absorbing $V$ and $Q$ into the control unitary. Let $B' := QBV$ and $C' := QCV$. Assume that $B'$ and $C'$ do not commute, and (wlog) that $\mathcal{A}$ is the computational basis (the same result can be obtained by writing $a$ and $a^\perp$ in place of 0 and 1 in what follows). Choose some eigenvector $\ket{\phi_1}\ket{\phi_2}$ of the circuit, and write $U\ket{\phi_1} = c\ket{0}+d\ket{1}$. Then the action of the circuit on this eigenvector is 
\[
\ket{\phi_1}\ket{\phi_2} = c\ket{0}\ket{\phi_2}+d\ket{1}\ket{\phi_2} \mapsto c\ket{0}B'\ket{\phi_2}+d\ket{1}C'\ket{\phi_2} \mapsto c P\ket{0}B'\ket{\phi_2}+d P\ket{1}C'\ket{\phi_2}.
\]
Since $P$ is unitary, $P\ket{0}$ and $P\ket{1}$ are orthogonal, and so the final state is only product if either $c = 0$ or $d = 0$, or if $B'\ket{\phi_2} \propto C'\ket{\phi_2}$. In the latter case, by Lemma \ref{lem:product}, $\ket{\phi_2}$ must be an eigenvector of both $B'$ and $C'$, which implies that $[B',C']=0$. By assumption, this is not the case, and so we must have that $c=0$ or $d=0$. 
This implies that $U = P^\dag$, and also that $\ket{\phi_2}$ is an eigenvector of at least one of $B'$ and $C'$. 
\\\\
Now we consider the case where $[B',C'] = 0$. In this case, we know from Section \ref{sec:defs} that $\CU{A}{B'}{C'} = \UC{E}{A}{A'}$, where $\mathcal{E}$ is the shared eigenbasis of $B'$ and $C'$ and $A, A'$ are as defined in Section \ref{sec:defs}. Moreover, we can absorb $U$ and $P$ into the control unitary, yielding $\UC{E}{PAU}{PA'U}$.
\\\\
Finally, if $B = e^{i\phi}C$ for some angle $\phi$, then from Section \ref{sec:defs} we know that the circuit collapses to two sets of 3 unitaries acting on each qubit separately.
\end{proof}
%%%%%%%%%%%%
The following corollary follows immediately from Lemma \ref{lem:single_2_qubit}, and demonstrates how to construct a single 2-qubit control unitary in each of the three cases above.
%%%%%%%%%%%%
\begin{corollary}
If the circuit from Lemma \ref{lem:single_qubit_gates} has a product eigenbasis, then it can be written as a single control unitary. 
\end{corollary}
\begin{proof}
The correctness follows from Lemma \ref{lem:single_2_qubit}. To find the correct form for the control unitary, we observe that if $[QCV,QBC]=0$, then we can simply absorb the unitaries $U, V, P, Q$ into $\CU{A}{B}{C}$ as in the second half of the proof of Lemma \ref{lem:single_qubit_gates}, yielding a control unitary $\UC{E}{A}{A'}$. If $B = e^{i\phi}C$ for some angle $\phi$, then we can write the entire circuit as two single-qubit unitaries $UAP \otimes QBV$, where $A = \unitary{1}{0}{0}{e^{i\phi}}$. Finally, if $[QCV,QBV]\neq 0$, then $U$ and $W$ must be diagonal in the $\mathcal{A}$ basis, and so they just contribute a relative phase $e^{i\theta}$ which can be absorbed into $B$ and $C$, yielding the control unitary $\CU{A}{e^{i\theta}QBV}{e^{i\theta}QCV}$
\end{proof}
%%%%%%%%%%%%

Occasionally, we might encounter circuits containing gates controlled on a number of qubits, and acting on a target qubit with a unitary that is diagonal in that qubit's associated basis. In these cases, we can replace the gate with an equivalent gate that is controlled on a different set of qubits, and that acts on a different target qubit, but still with a unitary that is diagonal in that qubit's basis -- see Figure \ref{fig:swap_targets}.

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.8]{diagrams/multi_control_final.pdf}
\caption{Changing the target qubit for a multi-controlled diagonal gate.}
\label{fig:swap_targets}
\end{center}
\end{figure}

%%%%%%%%%%%%
\begin{lemma}\label{lem:lem_3}
Suppose that we have an $n$-qubit circuit composed of a single target qubit $i$, with $n-1$ control unitaries acting on it, each controlled on different control lines (which can be controlled in different bases). Let the basis on the $k$th line be $\mathcal{B}_k = \{\ket{b^k_0}, \ket{b^k_1}\}$ (where $\ket{b^k_1}=\ketp{b^k_0}$). Let $x = x_1, x_2, \dots, x_{n-1}$ be an $(n-1)$-bit string, and $U^{(i)}_x$ be the unitary applied to qubit $i$ when the other control lines are in the state $\ket{x} = \ket{b^1_{x_1}} \otimes \ket{b^2_{x_2}} \otimes \cdots \otimes \ket{b^n_{x_{n-1}}}$. 

Further suppose that $U^{(i)}_x$ is diagonal (in the $\mathcal{B}_i$ basis) for all $x$. Then the circuit can be re-written as a control unitary acting on any qubit $j \in [n]$, controlled on all the others, such that the unitary $U^{(j)}$ acting on the new target qubit $j$ remains diagonal in the basis $\mathcal{B}_j$ of that qubit.
\end{lemma}
\begin{proof}
Let the eigenvalues of $\ket{b^0_0}\ket{x}$ and $\ketp{b^0_1}\ket{x}$ be $e^{i \theta_{0,x}} = e^{i \theta_{1,x_0,x_1,\dots,x_{n-1}}}$ and $e^{i \theta_{1,x_0,x_1,\dots,x_{n-1}}}$. 

Now let $\ket{y, 0}$ (resp. $\ket{y,1}$) be the state where all lines but the $j$th are in state $\ket{y}$, and the $j$th qubit is in state $\ket{b^j_0}$ (resp $\ket{b^j_1}$). That is, the qubits are in the state $\ket{b^0_{y_0}}\otimes \cdots \otimes \ket{b^j_{b}} \otimes \cdots \otimes \ket{b^n_{y_n}}$ for $b=0$ (resp. $b=1$). Then $B_y$ has eigenvalues $e^{i \theta_{y_1, \dots, 0_j, \dots, y_n}}$ and $e^{i \theta_{y_1, \dots, 1_j, \dots, y_n}}$ corresponding to eigenvectors $\ket{y,0}$ and $\ket{y,1}$, respectively. 

Hence, $B_y$ is diagonal in basis $\mathcal{B}_j$. Furthermore, given that one knows this condition is met, it is efficient to compute $B_y$ for any $y$.
\end{proof}
%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Building circuits from 1 and 2 qubit gates}
In what follows, we will prove that all circuits composed of 1- and 2-qubit gates that satisfy the product eigenbasis condition can be written in the form shown in Figure \ref{fig:main_structure}, and that a circuit of this form can be efficiently generated from the original circuit. We will now define what we mean by control, target, ambiguous, and free lines. 
%%%%%%%%%%%%
\begin{definition}\label{def:types_of_qubit}
We define the following types of qubit in our circuit:
\begin{itemize}
\item Control in $\mathcal{B}$ : Any line that is used to control the application of a control unitary on a target line, in the basis $\mathcal{B} = \{\ket{b}, \ketp{b}\}$. I.e. the action of the circuit on the target line is either $U_{0,x}$ or $U_{1,x}$, depending on whether the control line is in the state $\ket{b}$ or $\ketp{b}$, and all other control lines are in the state $\ket{x}$. Then there must exist some $x$ such that $[U_{0,x}, U_{1,x}] \neq 0$ (else this qubit would be an Ambiguous qubit). The basis of this line is fixed to be $\mathcal{B}$, and it can be acted upon by 2-qubit gates shared with control, target, and ambiguous lines. 
\item Target : Any line that is only acted upon only by control unitaries controlled by a control line.
\item Ambiguous in $\mathcal{B}$ : A line that has a associated basis $\mathcal{B}$, but is not an actual control line. It may be acted upon only by 2-qubit gates shared with other ambiguous lines and control lines, and may at some point in the circuit become a true control or a true target line.
\item Free : A line that is only acted upon by 1-qubit gates.
\end{itemize}
\end{definition}
%%%%%%%%%%%%

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=1.0]{diagrams/main_structure_alt_2.pdf}
\caption{\chris{Describe each type of gate / link it to previous descriptions}}
\label{fig:main_structure}
\end{center}
\end{figure}

% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[scale=1.0]{diagrams/main_structure_alt.pdf}
% \caption{Alternate figure: I think the notation for the $P_{\mathcal{A}\mathcal{B}}$-type gates is clearer, and reflects their nature? (this way they look more like a $CZ$ gate). I don't like the gate on the right though. I think it should be as in the original figure.}
% \label{fig:main_structure_alt}
% \end{center}
% \end{figure}


Whenever we add a 2-qubit gate $U$ to a circuit $C$, all qubits that have an associated basis (i.e. control, ambiguous, or free qubits) and aren't acted upon by this new gate remain unchanged. That is, in the eigenbasis of the new circuit $UC$, the basis associated to each of these qubits remains unchanged from the eigenbasis of the previous circuit $C$. The following lemma formalises this observation.
%%%%%%%%%%%%
\begin{lemma}\label{lem:4}
Suppose that we have a circuit $C$ on $n$ qubits in the control product form (see Figure \ref{fig:main_structure}). Now suppose that a 2-qubit gate $U$ is applied to qubits $i$ and $j$, and that the unitary of the resulting circuit has a product eigenbasis $\mathcal{P}$. 

Then for all qubits $k \neq i, j$ corresponding to control, ambiguous, or free lines in basis $\mathcal{B}_k$ (as defined in Definition \ref{def:types_of_qubit}), the $k$th qubit of every eigenvector in $\mathcal{P}$ is in the state $\ket{b^{(k)}_0}$ or $\ket{b^{(k)}_1}$ from $\mathcal{B}_k$.
\end{lemma}
\begin{proof}
Let $S$ be the set of all control, ambiguous, and free lines other than $i$ and $j$, and let $S' = [n]\setminus S$ be the rest. Let $x$ be an $|S|$-bit string, and suppose that all qubits in $S$ are in the state $\ket{x}_S := \bigotimes_{k \in S} \ket{b^{(k)}_{x_k}}$. For some state $\ket{\psi}$ on the qubits in $S'$, we have $\ket{\psi}_{S'}\otimes\ket{x}_S \mapsto^{C} \ket{\psi'}_{S'} \otimes \ket{x}_S$, and we can write the action of $C$ as
\[
C = \sum_{x \in \{0,1\}^{|S|}} (C_{x})_{S'} \otimes \proj{x}_S,
\]
where $(C_{x})_{S'}$ is a unitary acting on the qubits in $S'$. Let $\mathcal{U}\mathcal{C}_x$ be an eigenbasis for $UC_x$. Then $\bigcup_{x \in \{0,1\}^{|S|}} \left(\mathcal{U}\mathcal{C}_x \otimes \proj{x}_S\right)$ is an eigenbasis of $UC$, and is product if the basis $\mathcal{U}\mathcal{C}_x$ is product for all $x \in \{0,1\}^{|S|}$. 
\\\\
Suppose by way of contradiction that there is no such product eigenbasis for $UC_{x'}$, for some $x'$, but that there \emph{is} a product eigenbasis for the whole circuit $UC$. Choose an eigenvector $\ket{\phi}_{S'} \otimes \ket{\psi}_S$ from that basis, and write $\ket{\psi}_S = \sum_{x \in \{0,1\}^{|S|}} \alpha_x \ket{x}_S$. Note that there must exist some choice of $\ket{\phi}$ such that $\alpha_{x'} \neq 0$, else the set of eigenvectors wouldn't span the entire space over the $n$ qubits. Without loss of generality, assume that we have chosen such a $\ket{\phi}$. 

The circuit $UC$ acts on this eigenvector as 
\[
	\ket{\phi}_{S'} \otimes \ket{\psi}_S \mapsto \sum_{x \in \{0,1\}^{|S|}} \alpha_x \left( UC_{x}\ket{\phi}\right) \otimes \ket{x}_S \quad = \quad e^{i\theta} \ket{\phi}_{S'} \otimes \ket{\psi}_S
\]
for some angle $\theta$. 
By Lemma \ref{lem:product}, the equality can only be true if $\ket{\phi}$ is an eigenvector of all $UC_x$ such that $\alpha_x \neq 0$ (which includes $x'$ by assumption). Since this holds for any eigenvector that we choose from the eigenbasis of $UC$, this contradicts our assumption that there exists no product eigenbasis for $UC_x$. Hence there must exist a product eigenbasis for $UC$ whose eigenvectors are of the form $\ket{\phi}_{S'} \otimes \ket{x}_S$ for all $x \in \{0,1\}^{|S|}$. 

In particular, this means that for any qubit $k \neq i, j$ corresponding to a control, ambiguous, or free line in basis $\mathcal{B}$, the $k$th qubit of any eigenvector of the circuit $UC$ remains unchanged from the corresponding eigenvector of the circuit $C$.
\end{proof}
%%%%%%%%%%%%

The next lemma, and the corollary that follows, show what constraints must be obeyed by a new 2-qubit gate if it is to act on a control qubit $i$ in basis $\mathcal{A}$ and another qubit $j$. In general, the new unitary must be a control-unitary, controlled on qubit $i$ in basis $\mathcal{A}$ and acting on qubit $j$. However, if a certain condition is met, then it is possible for the gate to be a control-unitary of the form $\CU{E}{B}{B'}$ for some basis $\mathcal{E}$ and commuting unitaries $B$ and $B'$. In this case, by Lemma \ref{lem:4}, the gate can be controlled on either one of $i,j$, whilst acting on the other. 
%%%%%%%%%%%%
\begin{lemma}\label{lem:5}
Once again, suppose that we have a circuit $C$ on $n$ qubits in control product form, and that a 2-qubit gate $U$ is applied to qubits $i$ and $j$, and also that the unitary of the resulting circuit has a product eigenbasis.

Suppose that qubit $i$ is a control qubit in basis $\mathcal{A}$ (which for simplicity, and wlog, we will assume is just the computational basis). Then, either
\begin{itemize}
\item[(i)] There exists a product eigenbasis of $UC$ in which line $i$ always has state $\ket{0}_i$ or $\ket{1}_i$, or
\item[(ii)] Line $j$ is the only target line that $i$ acts on, and the following condition holds. Let all other control lines be in the state $\ket{x}$ and suppose that $C$ is such that $V_{0,x}$ is applied to $j$ when $i$ is in state $\ket{0}_i$, and $V_{1,x}$ is applied to $j$ when $i$ is in state $\ket{1}_i$. Then there exist unitaries $D_0$ and $D_1$ such that both $D_0V_{0,x}$ and $D_1V_{1,x}$ are diagonal in a basis $\mathcal{D}$ for all $x$. 
\end{itemize}
\end{lemma}
\begin{proof}
Similarly to the proof of Lemma \ref{lem:4}, we can consider the actions and eigenbases of the circuits $UC_x$ for $x \in \bit^{|S|}$, where $S$ is the set of all control, ambiguous, and free lines other than $i$ and $j$. Let $T$ be the set of all target qubits outside of $i$ and $j$. 
\\\\
First, suppose that there is at least one line $l$ in $T$ that $i$ acts as a control on. Let $W^{(t)}_{0,x}$ (resp. $W^{t}_{1,x}$) be the action of $U$ on qubit $t \in T$ when qubit $i$ is in state $\ket{0}_i$ (resp. $\ket{1}_i$). For an arbitrary (product) eigenvector $\ket{\psi}_i\ket{\phi}_j\ket{x}_{S}\ket{\varphi}_T$, then writing $\ket{\psi}_i = \alpha\ket{0}_i + \beta\ket{1}_i$, the action of $UC_x$ on this state is
\begin{eqnarray*}
	(\alpha\ket{0}_i + \beta\ket{1}_i)\ket{\phi}_j\ket{x}_S\ket{\varphi}_T 
	\mapsto 
	&\alpha U(\ket{0}_i V_{0,x} \ket{\phi}_j) \ket{x}_{S} W^{(1)}_{0,x} \otimes \cdots \otimes W^{(|T|)}_{0,x} \ket{\varphi}_T + \\
	&\beta U(\ket{1}_i V_{1,x} \ket{\phi}_j) \ket{x}_{S} W^{(1)}_{1,x} \otimes \cdots \otimes W^{(|T|)}_{1,x} \ket{\varphi}_T,
\end{eqnarray*}
Therefore, given that $\ket{\psi}_i\ket{\phi}_j\ket{x}_{S}\ket{\varphi}_T$ is an eigenvector of $UC_c$, then we must have 
\begin{eqnarray*}
&\alpha U(\ket{0}_i V_{0,x} \ket{\phi}_j) W^{(1)}_{0,x} \otimes \cdots \otimes W^{(|T|)}_{0,x} \ket{\varphi}_T& + \\
&\beta U(\ket{1}_i V_{1,x} \ket{\phi}_j) W^{(1)}_{1,x} \otimes \cdots \otimes W^{(|T|)}_{1,x} \ket{\varphi}_T&
= e^{i\theta}\ket{\psi}_i\ket{\phi}_j\ket{\varphi}_T.
\end{eqnarray*}
for some angle $\theta$. By Lemma \ref {lem:product}, this implies that $\ket{\phi}_T$ is an eigenvector of both $W^{(1)}_{0,x} \otimes \cdots \otimes W^{(|T|)}_{0,x}$ and $W^{(1)}_{1,x} \otimes \cdots \otimes W^{(|T|)}_{1,x}$ with eigenvalue $e^{i\theta}$. Since, by assumption, $\ket{\phi}$ is a product state $\ket{\phi^{(1)}} \otimes \ket{\phi^{(2)}} \otimes \cdots \otimes \ket{\phi^{(l)}} \otimes \cdots \otimes \ket{\phi^{(|T|)}}$, then $\ket{\phi^{(l)}}$ must be an eigenvector of both $W^{(l)}_{0,x}$ and $W^{(l)}_{1,x}$. This means that qubit $i$ does not act (non-trivially) as a control qubit on qubit $l$, contradicting our assumption above. Hence, there cannot be a qubit in $T$ that is acted upon as a control by $i$. 
\\\\
Henceforth we will assume that the only qubit that $i$ acts as a control on is $j$. Then the action of the circuit on the same eigenvector (omitting the $S$ (control) register) is 
\[
	\alpha U(\ket{0}_i V_{0,x} \ket{\phi}_j) \ket{\varphi}_T + \beta U(\ket{1}_i V_{1,x} \ket{\phi}_j) \ket{\varphi}_T   \quad \propto \quad   \ket{\psi}_i\ket{\phi}_j\ket{\varphi}_T.
\]
Assume $\alpha, \beta \neq 0$. Then because $U(\ket{0}_iV_{0,x}\ket{\phi}_j)$ and $U(\ket{1}_iV_{1,x}\ket{\phi}_j)$ are orthogonal, we can write $U(\ket{0}_iV_{0,x}\ket{\phi}_j) = \ket{u}_i\ket{\phi}_j$ and $U(\ket{1}_iV_{1,x}\ket{\phi})_j) = \ketp{u}_i\ket{\phi}_j$, for some state $\ket{u}$. But because $\{\ket{0}\ket{\phi}, \ket{1}\ket{\phi}, \ket{0}\ketp{\phi}, \ket{1}\ketp{\phi} \}$ forms an orthonormal basis for the two qubits, this implies that 
\[
	\ket{0}_i\ketp{\phi}_j \mapsto U(\ket{0}_iV_{0,x}\ketp{\phi}_j) = \ket{\tilde{u}}_i\ketp{\phi}_j
\]
\[
	\ket{1}_i\ketp{\phi}_j \mapsto U(\ket{1}_iV_{1,x}\ketp{\phi}_j) = \ketp{\tilde{u}}_i\ketp{\phi}_j
\]
for some state $\ket{\tilde{u}}$. 
\\\\
Define $E_x$ and $F_x$ by their actions on basis states: 
\[
\begin{matrix}
E_x\ket{0} = \ket{u} & \quad & F_x\ket{0} = \ket{\tilde{u}} \\
E_x\ket{1} = \ketp{u} & \quad & F_x\ket{1} = \ketp{\tilde{u}} 
\end{matrix},
\]
and let $\mathcal{D}$ be the basis $\{\ket{\phi}, \ketp{\phi}\}$. Then $U(\CU{A}{V_{0,x}}{V_{1,x}}) = \UC{D}{E_x}{F_x}$, implying that we can decompose $U$ as 
\[
	U = \CU{A}{V^\dag_{0,x}}{V^\dag_{1,x}} \UC{D}{E_x}{F_x},
\]
(See Figure \ref{fig:lem_5_proof} for clarity.) 
\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=1.0]{diagrams/lem_5_proof.pdf}
\caption{$U(\CU{A}{V_{0,x}}{V_{1,x}}) = \CU{O}{E}{F}$ implies that $U = \CU{A}{V^\dag_{0,x}}{V^\dag_{1,x}} \CU{O}{E}{F}$.}
\label{fig:lem_5_proof}
\end{center}
\end{figure}

We require the circuit $UC_x$ to have a product eigenbasis for all $x$. In particular, the circuit formed by applying $U$ after $\CU{A}{V_{0,x'}}{V_{1,x'}}$ must have a product eigenbasis. Restricting our attention to qubits $i$ and $j$, the unitary acting on these two qubits must be a control unitary (by Lemma \ref{lem:single_2_qubit}). As we have just shown, this circuit can be written as  $\CU{A}{V^\dag_{0,x}V_{0,x'}}{V^\dag_{1,x}V_{1,x'}} \UC{D}{E_x}{F_x}$.
\\\\
In the case $[E_x,F_x]\neq 0$, then both $V^\dag_{0,x}V_{0,x'}$ and $V^\dag_{1,x}V_{1,x'}$ must be diagonal in the $\mathcal{D}$ basis for all $x,x'$, allowing us to re-write the circuit as a single control unitary, which can be controlled on either of the 2 qubits by Lemma \ref{lem:lem_3}.
\\\\
In the case that $[E,F]=0$, they must be diagonal in the same basis. Supposing that this basis is $\mathcal{B}$, then the circuit can be written as $\CU{A}{V^\dag_{0,x}V_{0,x'}}{V^\dag_{1,x}V_{1,x'}} \CU{B}{D}{D'}$ for some $D, D'$ such that $[D,D']=0$, which is only a valid control-unitary (which indeed it must be, by Lemma \ref{lem:single_2_qubit}) if $\mathcal{A} = \mathcal{B}$. This circuit has an eigenbasis with the $i$th qubit always set to $\ket{0}_i$ or $\ket{1}_i$ (since the basis of qubit $i$ must be $\mathcal{A}$). 
\\\\
In summary, if $i$ is a control line, then $j$ can be its only target, and applying a unitary $U$ to $i$ and $j$ either yields a unitary with an eigenbasis in which the $i$th line is always $\ket{0}_i$ or $\ket{1}_i$, or else $V^\dag_{0,x}V_{0,x'}$ and $V^\dag_{1,x}V_{1,x'}$ are diagonal in basis $\mathcal{D}$ for all $x,x'$, and the unitary $U$ is of the form $\CU{A}{V^\dag_{0,x}V_{0,x'}}{V^\dag_{1,x}V_{1,x'}} \CU{B}{D}{D'}$ for some fixed $x$ and commuting unitaries $D, D'$. Choosing $D_0 = V^\dag_{0,x}$ and $D_1 = V^\dag_{1,x}$ suffices to prove the result. 

\end{proof}
%%%%%%%%%%%%


%%%%%%%%%%%%
\begin{corollary}\label{cor:2}
Except in case (ii) of Lemma \ref{lem:5}, the unitary $U$ applied to the circuit must be a control unitary, controlled by qubit $i$ and acting on qubit $j$. 
\end{corollary}
\begin{proof}
As before, consider the eigenbasis of $UC_x$ for some $x$. We know that in the case we are considering, any eigenvector from this basis has either $\ket{0}_i$ or $\ket{1}_i$ on the $i$th line. Without loss of generality, choose an eigenvector with a $\ket{0}$ on this qubit: $\ket{0}_i\ket{\psi}_j\ket{x}_S\ket{\phi}_T$. The action of the circuit on this state is 
\begin{eqnarray*}
	\ket{0}_i\ket{\psi}_j\ket{x}_S\ket{\phi}_T &\mapsto& \ket{0}_i V_{0,x}\ket{\psi}_j \ket{x}_S W_{0,x}\ket{\phi}_T \\
	&\mapsto& U(\ket{0}_i V_{0,x}\ket{\psi}_j) \ket{x}_S W_{0,x}\ket{\phi}_T \\
	&=& e^{i\varphi} \ket{0}_i\ket{\psi}_j\ket{x}_S\ket{\phi}_T
\end{eqnarray*}
for some angle $\varphi$.
This implies that $\ket{\phi}_T$ is an eigenvector of $W_{0,x}$. Moreover, $\ket{0}_i\ketp{\psi}_j\ket{x}_S\ket{\phi}_T$ must also be an eigenvector of $UC_x$, as must $\ket{1}_i\ket{\theta}_j\ket{x}_S\ket{\phi}_T$ and $\ket{1}_i\ketp{\theta}_j\ket{x}_S\ket{\psi}_T$, for some $\ket{\theta}$. This implies that $U = \proj{0}_i \otimes B + \proj{1}_i \otimes C = \CU{A}{B}{C}$ , with $\ket{\psi}, \ketp{\psi}$ eigenvectors of $BV_{0,x}$ and $\ket{\theta}, \ketp{\theta}$ eigenvectors of $CV_{1,x}$.
\end{proof}
%%%%%%%%%%%%

The results so far can be summed up by the following theorem. 
%%%%%%%%%%%%
\begin{theorem}
Applying a 2-qubit gate $U$ to qubits $i$ and $j$ after applying the circuit $C$, whilst maintaining that the final circuit $UC$ has a product eigenbasis, places the following constraints on $U$:

\begin{table}[h]
\hspace{-1.5cm}
\begin{tabular}{llll}
\multicolumn{1}{c}{$i$}          & \multicolumn{1}{c}{$j$}                              & \multicolumn{1}{c}{$U$}                       & \multicolumn{1}{c}{Proof}                                                         \\ \hline
Control with basis $\mathcal{A}$ & Control with basis $\mathcal{B}$                     & Diagonal in $\mathcal{A} \otimes \mathcal{B}$ & ?                                                                                 \\
Control with basis $\mathcal{A}$ & Ambiguous (with basis $\mathcal{B}$)                 & Control unitary in basis $\mathcal{A}$        & ?                                                                                 \\
Control with basis $\mathcal{A}$ & Free                                                 & Control unitary in basis $\mathcal{A}$        & \begin{tabular}[c]{@{}l@{}}Lemma \ref{lem:5}\\ Corollary \ref{cor:2}\end{tabular} \\
Control with basis $\mathcal{A}$ & Target (Except in special case of Lemma \ref{lem:5}) & Control unitary in basis $\mathcal{A}$        & \begin{tabular}[c]{@{}l@{}}Lemma \ref{lem:5}\\ Corollary \ref{cor:2}\end{tabular}
\end{tabular}
\end{table}
\end{theorem}
%%%%%%%%%%%%

We now deal with the constraints placed on gates that act on ambiguous qubits. 

%%%%%%%%%%%%
\begin{lemma}\label{lem:7}
Suppose that the circuit $C$ has already been applied, and now a 2-qubit gate $U$ is applied to qubits $i$ and $j$, which are both ambiguous in bases $\mathcal{A}$ and $\mathcal{B}$, respectively. Then in order for $UC$ to have a product eigenbasis, $U$ must be a control unitary controlled on either $i$, in basis $\mathcal{A}$; $j$, in basis $\mathcal{B}$; or both. 
\end{lemma}
\begin{proof}
Once again, we will consider the action of the circuit $UC_x$ for some $x$. We know that so far all gates will have acted on line $i$ in basis $\mathcal{A}$ and line $j$ in basis $\mathcal{B}$. There may also have been some unitaries acting between them of the form $\CU{A}{B}{B'}$ (for commuting $B, B'$), which we can combine into a single gate $P_{{\mathcal{A}\mathcal{B}}_x}$ diagonal in $\mathcal{A} \otimes \mathcal{B}$. The resulting circuit $UC_x$, when restricting attention to qubits $i$ and $j$, is $U P_{{\mathcal{A}\mathcal{B}}_x}$. Since this circuit is promised to have a product eigenbasis, it must be of control-unitary form, which (wlog) we will write as $\CU{E}{H_x}{K_x}$. This implies that 
$U = \CU{E}{H_x}{K_x} {{P_{\mathcal{A}\mathcal{B}}}_x}^\dag$ (see Figure \ref{fig:ambiguous_full} for clarity).

\begin{figure}
\hspace{-2cm}
    \includegraphics[scale=1.0]{diagrams/amgibuous_full.pdf}
    \caption{$U P_{{\mathcal{A}\mathcal{B}}_x} = \CU{E}{H_x}{K_x}$ implies that $U = \CU{E}{H_x}{K_x} {{P_{\mathcal{A}\mathcal{B}}}_x}^\dag$}    \label{fig:ambiguous_full}
\end{figure}

But since the condition must hold for other values of $x$, this implies that for all $x' \neq x$, 
$UC_{x'} = \CU{E}{H_x}{K_x} {{P_{\mathcal{A}\mathcal{B}}}_x}^\dag {{P_{\mathcal{A}\mathcal{B}}}_{x'}}^\dag.$ (shown in Figure \ref{fig:ambiguous_4} for clarity).
If $P_{{\mathcal{A}\mathcal{B}}_x} = P_{{\mathcal{A}\mathcal{B}}_{x'}}$ for all $x,x'$, then these cancel, and we have $U = \CU{E}{H_x}{K_x}$. 

\begin{figure}
\centering
    \includegraphics[scale=1.0]{diagrams/ambiguous_4.pdf}
    \caption{$\CU{E}{H_x}{K_x} {{P_{\mathcal{A}\mathcal{B}}}_x}^\dag {{P_{\mathcal{A}\mathcal{B}}}_{x'}}^\dag.$}    \label{fig:ambiguous_4}
\end{figure}

Otherwise, the two unitaries $P_{{\mathcal{A}\mathcal{B}}_{x}}$ and $P_{{\mathcal{A}\mathcal{B}}_{x'}}$ will combine to form some circuit $\CU{E}{H_x}{K_x} {P_{{\mathcal{A}\mathcal{B}}_{x}}}^\dag P_{{\mathcal{A}\mathcal{B}}_{x'}} =: \CU{E}{H_x}{K_x} P_{{\mathcal{A}\mathcal{B}}_{xx'}}$, which must have a product eigenbasis and therefore be a control-unitary itself (by Lemma \ref{lem:single_2_qubit}). We can write the unitary $P_{{\mathcal{A}\mathcal{B}}_{xx'}}$ in control-unitary form as $\CU{A}{P_{{\mathcal{A}\mathcal{B}}_{xx'}}^{(a)}}{P_{{\mathcal{A}\mathcal{B}}_{xx'}}^{(a^\perp)}}$, where ${P_{{\mathcal{A}\mathcal{B}}_{xx'}}^{(b)}}$ is the action of $P_{{\mathcal{A}\mathcal{B}}_{xx'}}$ on qubit $j$ when qubit $i$ is in state $\ket{b} \in \{\ket{a},\ketp{a}\}$. For this circuit to be a valid control unitary, then either $\mathcal{A} = \mathcal{E}$, or $H_x$ and $K_x$ are diagonal in $\mathcal{B}$, or both. 

In the first case, for some $x'$, the resulting circuit must be a control-unitary of the form $\CU{A}{U^{(a)}_{x'}}{U^{(a^\perp)}_{x'}}$. In the second case, where $H_x$ and $K_x$ are diagonal in $\mathcal{B}$, then the circuit is of the form $\UC{B}{U^{(b)}_{x'}}{U^{(b^\perp)}_{x'}}$, where in both cases we define $U^{(a)}_{x'} = H_x P_{{\mathcal{A}\mathcal{B}}_{xx'}}$, and the others are defined similarly. If both $H_x$ and $K_x$ are diagonal in $\mathcal{B}$, and $\mathcal{E}=\mathcal{A}$, then the circuit is of the form $\CU{A}{B}{B'}$ for commuting $B, B'$, and the qubits $i$ and $j$ remain ambiguous in bases $\mathcal{A}$ and $\mathcal{B}$, respectively.

If, instead, only one of the conditions holds, then if $[U^{(a)}_{x}, U^{(a^\perp)}_{x}] \neq 0$ for all $x$, then the control line (which is either $i$ or $j$ above) becomes a true control line in basis $\mathcal{A}$ (as per Definition \ref{def:types_of_qubit}), and the target line becomes a true target line. Otherwise, qubits $i$ and $j$ remain ambiguous in their respective bases. 
\end{proof}
%%%%%%%%%%%%

The remaining cases can be summarised by the following theorem.
%%%%%%%%%%%%
\begin{theorem}\label{lem:10}
Applying a 2-qubit gate $U$ to qubits $i$ and $j$, after applying the circuit $C$, whilst maintaining that the final circuit $UC$ has a product eigenbasis places the following constraints on $U$:

\begin{table}[h]
\begin{tabular}{c|c|c}
$i$    & $j$                        & $U$                                                                                                                                           \\ \hline
Target & Target                     & \begin{tabular}[c]{@{}c@{}}Does not exist unless \\ condition (i) below is satisfied\end{tabular}                                               \\
Target & Free                       & \begin{tabular}[c]{@{}c@{}}Control on $j$ in any basis\\ (Or control on $i$ if condition (ii) below is satisfied)\end{tabular}                   \\
Target & Ambiguous in $\mathcal{B}$ & \begin{tabular}[c]{@{}c@{}}Control on $j$ in basis $\mathcal{B}$\\ (Or a control in any basis if condition (iii) below is satisfied)\end{tabular} \\
Free   & Free                       & Control on either $i$ or $j$, in any basis.                                                                                                  
\end{tabular}
\end{table}

\end{theorem}
\begin{proof}
In all of the above cases, we can assume that there have been no unitaries acting between qubits $i$ and $j$ so far (else, as we will see, none of the above cases will exist). Therefore we can view the circuit $C_x$ so far as acting with a unitary $W_x$ on qubit $i$ and a unitary $V_x$ on qubit $j$ (in some cases the dependence on $x$ will be redundant). 

Similarly to before, we can make the following set of claims. The (2-qubit) unitary acting on qubits $i$ and $j$ after applying the new gate $U$ must have a product eigenbasis, and therefore be a control unitary (by Lemma \ref{lem:single_2_qubit}). Writing this control unitary as $\CU{A}{B_x}{C_x}$, we must have that $U (W_x \otimes V_x) = \CU{A}{B_x}{C_x}$, and therefore $U = \CU{A}{B_x}{C_x} (W^\dag_x \otimes V^\dag_x)$. Once again, the product eigenbasis condition must hold for other values of $x$. In particular, for any $x'$, we must have that $\CU{A}{B}{C} (W^\dag_x \otimes V^\dag_x) (W_{x'} \otimes V_{x'})$ is a control unitary. 

If $[B_x, C_x] \neq 0$, then Lemma \ref{lem:single_qubit_gates} implies that $W^\dag_x W_{x'}$ is diagonal in basis $\mathcal{A}$ for all $x, x'$. If $[B_x, C_x] = 0$ for all $x, x'$ (and hence share an eigenbasis $\mathcal{B}$), then either $W^\dag_x W_{x'}$ is diagonal in basis $\mathcal{A}$, or $V^\dag_x V_{x'}$ is diagonal in basis $\mathcal{B}$. If both unitaries are diagonal in their respective bases, then $UC_x$ acts as two single-qubit gates on both $i$ and $j$. 
\\\\
Now we deal with the specific cases stated in the theorem. 
\paragraph{Case 1 -- target : target} As we just saw, $UC$ can only have a product eigenbasis if, for all $x, x'$, either $W^\dag_x W_{x'}$ or $V^\dag_x V_{x'}$ is diagonal in some basis $\mathcal{A}$ or $\mathcal{B}$, respectively. This is condition (i) referenced in the statement of the theorem. In these cases, $U$ can act as a control unitary controlled on the basis $\mathcal{A}$ or $\mathcal{B}$. 

\paragraph{Case 2 -- target : free} The action of the circuit $C$ can be written as a tensor product of one unitary that depends on the other control lines in some way, $W_x$, and a single qubit unitary that depends on no other qubits, $V$. I.e. $C = W_x \otimes V$. Then $UC$ can have a product eigenbasis if $U$ acts as $(I\otimes V)\UC{E}{A}{B}$ for any basis $\mathcal{E}$ and 2-qubit unitaries $A, B$. 

If condition (ii) is satisfied -- $W^\dag_x W_{x'}$ is diagonal in some basis $\mathcal{A}$ for all $x, x'$ -- then $U$ may also act as a control unitary $\CU{A}{B}{C}$ for any 2-qubit unitaries $B, C$.  

\paragraph{Case 3 -- target : ambiguous} In this case, line $j$ has an associated basis $\mathcal{B}$. $UC$ has a product eigenbasis if $U$ acts as a control unitary controlled on basis $\mathcal{B}$ (i.e. is of the form $\UC{B}{A}{B}$ for any 2-qubit unitaries $A,B$). 

If condition (iii) is satisfied -- $W^\dag_x W_{x'}$ is diagonal in basis $\mathcal{A}$ for all $x, x'$ -- then $U$ can act as a control unitary controlled on basis $\mathcal{A}$ (i.e. is of the form $\CU{A}{B}{C}$ for any 2-qubit unitaries $B,C$). \chris{If $B^\dag_x B_{x'} = I$ for all $x,x'$, then we are in case 2 above. }

\paragraph{Case 4 -- free : free} In this case, the circuit so far has acted as $C = W \otimes V$, for $W, V$ 2-qubit unitaries independent of the state of the other qubits. Then $UC$ has a product eigenbasis if $U$ acts as $(W^\dag \otimes V^\dag)$ followed by a control unitary in any basis, controlled on either $i$ or $j$ (or both if it acts as a control unitary from $\mathcal{P}$ or $\mathcal{S}$). 
\end{proof}
%%%%%%%%%%%%
